High-throughput search for topological magnon materials

Topological magnons give rise to possibilities for engineering novel spintronics devices with critical applications in quantum information and computation, due to its symmetry-protected robustness and low dissipation. However, to make reliable and systematic predictions about material realization of topological magnons has been a major challenge, due to the lack of neutron scattering data for most materials. In this work, we significantly advance the symmetry-based approach for identifying topological magnons through developing a fully automated algorithm, utilizing the theory of symmetry indicators, that enables a highly efficient and large-scale search for candidate materials hosting field-induced topological magnons. This progress not only streamlines the discovery process but also expands the scope of materials exploration beyond previous manual or traditional methods, offering a powerful tool for uncovering novel topological phases in magnetic systems. Performing a large-scale search over all 1649 magnetic materials in Bilbao Crystallographic Server with a commensurate magnetic order, we discover 387 candidate materials for topological magnons, significantly expanding the pool of topological magnon materials. We further discuss examples and experimental accessibility of the candidate materials, shedding light on future experimental realizations of topological magnons in magnetic materials.

==> ExperimentalTable.tex <==


\hspace*{-2.6cm}
\begin{longtable}
{|p{0.15\textwidth}|p{0.85\textwidth}|}
\hline
\textbf{Category} & \textbf{Materials} \\
\hline
\endfirsthead

\hline
\textbf{Category} & \textbf{Materials} \\
\hline
\endhead

\hline
\endfoot

\hline
\caption{Chemical categories of some synthesis-\textit{relevant} topological magnon materials identified in this work with a nontrivial $\mathbb{Z}_4$ inversion index upon breaking into one of the magnetic subgroups (\textit{e.g.} $P\bar{1}$, $P2^\prime_1/c^\prime$, $C2^\prime/m^\prime$, $C2^\prime/c^\prime$, ..\textit{etc}) of their respective $\mathcal{MSG}s$. Such values diagnose either gapless Weyl magnons or gapped magnon axion insulator states depending on the $\mathcal{MSG}$ of the chosen material and possibly the details of the magnetic interactions between spins therein.}



\endlastfoot

% Transition metal magnets
\textbf{I- Transition Metal Magnets} & \\
\textit{IA- Transition Metal Insulators} & $\alpha$-Fe$_2$O$_3$, CoO, MnTe$_2$, NiFe$_2$O$_4$, NiCr$_2$O$_4$, MnV$_2$O$_4$, CdYb$_2$S$_4$, CdYb$_2$Se$_4$, MnPb$_4$Sb$_6$S$_{14}$, FePb$_4$Sb$_6$S$_{14}$, Ba$_2$CoO$_2$Ag$_2$Se$_2$, Sr$_2$CoO$_2$Ag$_2$Se$_2$, Sr$_2$Fe$_3$S$_2$O$_3$, BaCoSO, Sr$_3$ZnIrO$_6$, Ca$_4$IrO$_6$, Ca$_3$LiRuO$_6$, Sr$_3$LiRuO$_6$, Sr$_3$NaRuO$_6$, SrFeO$_2$, Ca$_3$LiOsO$_6$, Ca$_2$MnGaO$_5$, CuSb$_2$O$_6$, Cr$_2$ReO$_6$, Ca$_2$Fe$_2$O$_5$, Mn$_3$TeO$_6$, FeTa$_2$O$_6$, GeNi$_2$O$_4$, LiMnAs, CsMnP, CsMnBi, RbMnAs, RbMn, RbMnP, KMnP, KMnAs, RbMnAs, RbMnBi \\
\hdashline
\textit{IB- Metallic TM Pnictogens and Chalcogens} & CrN, Li$_{0.5}$FeCr$_{1.5}$S$_4$, FeCr$_2$S$_4$, SrMnSb$_2$, CoNb$_3$S$_6$, CsCo$_2$Se$_2$, CaCo$_{1.86}$As$_2$, Sr$_2$Cr$_3$As$_2$O$_2$, CuSe$_2$O$_5$ \\
\hdashline
\textit{IC- Metal to Insulator Transition Compounds} & NiS$_2$, KCuMnS$_2$, USb \\
\hdashline
\textit{ID- Transition Metal Intermetallics} & MnPt$_{0.5}$Pd$_{0.5}$, Mn$_3$Pt, MnCoGe, Mn$_5$Si$_3$, Fe$_{0.7}$Mn$_{0.3}$, Ni$_{1.64}$Co$_{0.36}$Mn$_{1.28}$Ga$_{0.72}$, Mn$_3$Sn$_2$, PrMnSi$_2$, CaFe$_4$Al$_8$, FeGe, FeSn, FeSn$_2$, FeGe$_2$, Mn$_3$Cu$_{0.5}$Ge$_{0.5}$N, Mn$_3$GaN, Mn$_3$ZnN, Mn$_3$GaC, Mn$_3$CuN, Mn$_2$As, Fe$_2$As, Cr$_2$As, EuFe$_2$As$_2$ \\
\hline
% f-block magnets
\textbf{II- f-block Magnets} & \\
\textit{IIA- Insulating f-block Magnets} & UO$_2$, NpSe, NpS, DyOCl, HoP, La$_3$OsO$_7$, La$_{2.8}$Ca$_{0.2}$OsO$_7$, Cd$_2$Os$_2$O$_7$, Ho$_2$Ru$_2$O$_7$, Er$_2$Ru$_2$O$_7$, Dy$_3$Al$_5$O$_{12}$, Tb$_3$Al$_5$O$_{12}$, Ho$_3$Al$_5$O$_{12}$, Er$_3$Ga$_5$O$_{12}$, Dy$_3$Ga$_5$O$_{12}$, Tb$_3$Ga$_5$O$_{12}$, Ho$_3$Ga$_5$O$_{12}$, Ln$_3$Tr$_5$O$_{12}$, Tm$_2$Mn$_2$O$_7$, Ho$_2$CrSbO$_7$, Ho$_2$Ru$_2$O$_7$, Er$_2$Ti$_2$O$_7$, Gd$_2$Sn$_2$O$_7$, Er$_2$Pt$_2$O$_7$, Er$_2$Sn$_2$O$_7$, Gd$_2$Ti$_2$O$_7$, Nd$_2$Sn$_2$O$_7$, Nd$_2$Hf$_2$O$_7$, Nd$_2$Zr$_2$O$_7$, Nd$_2$ScNbO$_7$, Sm$_2$Ti$_2$O$_7$, Tb$_2$Sn$_2$O$_7$, Yb$_2$Ti$_2$O$_7$, Yb$_2$Sn$_2$O$_7$ \\
\hdashline
\textit{IIB- Metallic f-block Pnictogens and Chalcogens} & UP, USb$_2$, UP$_2$, UGeS, UGeTe, NpBi, NpTe, NdCoAsO, LaCrAsO, CeCo$_2$P$_2$, CeSbTe \\
\hdashline
\textit{IIC- f-block Intermetallics} & Ho(Co$_{0.66}$Ga$_{0.33}$)$_2$, CeIr(In$_{0.97}$Cd$_{0.03}$)$_5$, ErNiGe, NdCo$_2$, GdMg, Pr$_2$Pd$_2$In, NdZn, Ho$_3$NiGe$_2$, Pr$_3$CoGe$_2$, Tb$_{0.6}$Y$_{0.4}$RhIn$_5$, NdMg, NdPt, TbPd$_{2.05}$Sn$_{0.95}$, Ho$_3$Ge$_4$, NdNiMg$_{15}$, Er$_3$Ge$_4$, Ce$_2$Ni$_3$Ge$_5$, HoRh, Yb$_2$Pd(In$_{0.4}$Sn$_{0.6}$), NdPd$_5$Al$_2$, ErFe$_2$Si$_2$, NdScSiC$_{0.5}$H$_{0.2}$, UNiGa$_5$, UPd$_2$Ge$_2$, URh$_3$Si$_5$, NpNiGa$_5$, U$_2$Pd$_{2.35}$Sn$_{0.65}$, ErMn$_2$Ge$_2$, YMn$_2$Si$_2$, YMn$_2$Si$_2$, YMn$_2$Ge$_2$, EuMn$_2$Si$_2$, CeMn$_2$Si$_2$, NdMn$_2$Si$_2$, NdMn$_2$Si$_2$, CeMn$_2$Si$_2$, CeMn$_2$Si$_2$, PrMn$_2$Si$_2$, PrMn$_2$Si$_2$, ErMn$_2$Ge$_2$, ErMn$_2$Ge$_2$, ErMn$_2$Si$_2$, ErMn$_2$Si$_2$, TbMn$_2$Si$_2$, DyCu, TbPt, TbPt$_{0.8}$Cu$_{0.2}$, NdSi, DyPt, TmNi, PrSi, NdNi$_{0.6}$Cu$_{0.4}$, HoNi, HoPt, ErPt, TmPt, Tb$_2$CoGa$_8$, Dy$_2$CoGa$_8$, Nd$_2$RhIn$_8$, U$_2$Rh$_2$Sn, U$_2$Ni$_2$Sn, CeRh$_2$Si$_2$, CeRu$_2$Al$_{10}$, U$_2$Ni$_2$In, YbCo$_2$Si$_2$ \\
\hline
% Structurally distinct
\textbf{III- Structurally Distinct} & \\
\textit{IIIA- Perovskite oxides and their derivatives} & BiCrO$_3$,TbCr$_{0.5}$Mn$_{0.5}$O$_3$,Lu$_{0.6}$Mn$_{0.4}$MnO$_3$,Pb$_{0.7}$Bi$_{0.3}$Fe$_{0.762}$W$_{0.231}$O$_3$, Pb$_{0.8}$Bi$_{0.2}$Fe$_{0.728}$W$_{0.264}$O$_3$, Nd$_2$CuO$_4$,Sr$_2$IrO$_4$,Nd$_2$NiO$_4$,Ca$_2$RuO$_4$,La$_2$NiO$_4$,LaSr$_3$Fe$_3$O$_9$, CaCu$_3$Fe$_2$Sb$_2$O$_{12}$,Sr$_2$CoOsO$_6$,Sr$_2$FeOsO$_6$, Cu$_3$Ni$_2$SbO$_6$, Bi$_2$RuMnO$_7$, NdFeO$_3$, CeFeO$_3$, TbFeO$_3$, SmFeO$_3$, NaOsO$_3$, LaCrO$_3$, YCrO$_3$, LaMnO$_3$, ErCrO$_3$, TmCrO$_3$, YRuO$_3$, PrMnO$_3$, Pr$_{0.95}$K$_{0.05}$MnO$_3$, NdMnO$_3$, KMnF$_3$, NdMnO$_3$, (CH$_3$NH$_3$)(Co(COOH)$_3$), Ho$_{0.2}$Bi$_{0.8}$FeO$_3$, Ho$_{0.15}$Bi$_{0.85}$FeO$_3$, La$_{0.875}$Ba$_{0.125}$Mn$_{0.875}$Ti$_{0.125}$O$_3$, La$_{0.90}$Ba$_{0.10}$Mn$_{0.90}$Ti$_{0.10}$O$_3$, La$_{0.95}$Ba$_{0.05}$Mn$_{0.95}$Ti$_{0.05}$O$_3$, La$_{0.95}$Ba$_{0.05}$MnO$_3$, LaMnO$_3$, YCr$_{0.5}$Mn$_{0.5}$O$_3$, SmFeO$_3$, SrRuO$_3$, TbCrO$_3$, DyCrO$_3$, TeNiO$_3$, YVO$_3$, LaSrFeO$_4$, Nd$_2$CuO$_4$, Pr$_2$CuO$_4$, LaSrFeO$_4$, LaCaFeO$_4$, LaBaFeO$_4$, La$_{0.75}$Bi$_{0.25}$Fe$_{0.5}$Cr$_{0.5}$O$_3$, LaCrO$_3$, CeFeO$_3$, InCrO$_3$, TlCrO$_3$, ScCrO$_3$, La$_2$NiO$_4$, Nd$_2$NiO$_4$, La$_2$CoO$_4$, Gd$_2$CuO$_4$, Sm$_2$CuO$_4$, Eu$_2$CuO$_4$, Bi$_{0.8}$La$_{0.2}$Fe$_{0.5}$Mn$_{0.5}$O$_3$, PrCrO$_3$, SmCrO$_3$, NdMn$_{0.8}$Fe$_{0.2}$O$_3$, Bi$_{0.8}$La$_{0.2}$Fe$_{0.5}$Mn$_{0.5}$O$_3$, PrCrO$_3$, SmCrO$_3$, NdMn$_{0.8}$Fe$_{0.2}$O$_3$, Rb$_2$Fe$_2$O(AsO$_4$)$_2$, NdMnO$_3$, NdMn$_{0.8}$Fe$_{0.2}$O$_3$, Pr$_{0.5}$Sr$_{0.5}$CoO$_3$, Pr$_{0.5}$Sr$_{0.4}$Ba$_{0.1}$CoO$_3$,Pr$_{0.5}$Sr$_{0.5}$MnO$_3$,(Tm$_{0.7}$Mn$_{0.3}$)MnO$_3$, (Ho$_{0.8}$Mn$_{0.2}$)MnO$_3$, Tb$_{0.55}$Sr$_{0.45}$MnO$_3$, Tb$_{0.55}$Sr$_{0.45}$MnO$_3$, SmCrO$_3$, TbFeO$_3$, Sc$_2$NiMnO$_6$, La$_2$CoPtO$_6$, Ca$_2$Fe$_{0.875}$Cr$_{0.125}$GaO$_5$ \\
\hdashline
\textit{IIIB- Halides and oxyhalides} & KNiF$_3$, KMnF$_3$, FeF$_3$, LiCoF$_4$, NaMnF$_4$, Na$_2$NiFeF$_7$, CsMn$_2$F$_6$, Fe$_2$F$_5$(H$_2$O)$_2$, Cr$_2$F$_5$, CsMnF$_4$, TlMnF$_4$, Na$_2$NiCrF$_7$, CsCoCl$_3$(D$_2$O)$_2$, CsNiF$_3$, SrFeO$_2$F, La$_2$NiO$_3$F$_2$, La$_{0.5}$Sr$_{0.5}$FeO$_{0.5}$F$_{0.5}$, Mn$_2$SeO$_3$F$_2$, Cu$_3$Mg(OD)$_6$Br$_2$, La$_2$NiO$_3$F$_{1.93}$ \\
\hdashline
\textit{IIIC- Polyatomic oxides (Sulfates,Phosphates, Carbonates,Vanadates, germanates and silicates)} & NiSO$_4$, FeSO$_4$, CoSO$_4$, FeSO$_4$F, FeOH$_4$, Li$_2$Fe(SO$_4$)$_2$, NaFeSO$_4$F, NaCoSO$_4$F, Co$_3$(PO$_4$)$_2$, CuFe$_2$(P$_2$O$_7$)$_2$, Fe$_2$MnBO$_5$, AgMnVO$_4$, VPO$_4$, Na$_3$Co(CO$_3$)$_2$Cl, Na$_2$BaMn(VO$_4$)$_2$, MnCO$_3$, NiCO$_3$, CoCO$_3$, Cu$_3$Y(SeO$_3$)$_2$O$_2$Cl,Cu$_3$Bi(SeO$_3$)$_2$O$_2$Br, (NH$_2$(CH$_3$)$_2$)(FeMn(HCOO)$_6$), (CH$_3$NH$_3$)Co(COOH)$_3$, (NH$_2$(CH$_3$)$_2$)(FeCo(HCOO)$_6$), NH$_4$FeCl$_2$(HCOO), [C(ND$_2$)$_3$]Mn(DCOO)$_3$, KFe$_3$(SO$_4$)$_2$(OH)$_6$, NaFe$_3$(SO$_4$)$_2$(OH)$_6$, AgFe$_3$(SO$_4$)$_2$(OD)$_6$, FeBO$_3$, CoFePO$_5$, NaFePO$_4$, Na$_2$BaFe(VO$_4$)$_2$, LaMn$_3$V$_4$O$_{12}$, ZrCo$_2$Ge$_4$O$_{12}$, CeCo$_2$Ge$_4$O$_{12}$, CeMnCoGe$_4$O$_{12}$, ZrMn$_2$Ge$_4$O$_{12}$, GdFeZnGe$_4$O$_{12}$, ErFeCuGe$_4$O$_{12}$, NaCeGe$_2$O$_6$, Fe$_4$Si$_2$Sn$_7$O$_{16}$, Mn$_2$SiO$_4$, Mn$_2$GeO$_4$, CuCl(C$_4$H$_4$N$_2$)$_2$(BF$_4$), CuBr(C$_4$H$_4$N$_2$)$_2$(BF$_4$) \\

\end{longtable}

==> NewExperimentalTable.tex <==
\hspace*{-2.6cm}
\begin{longtable}{|p{0.15\textwidth}|p{0.85\textwidth}|} 
\caption{Chemical categories of some synthesis-relevant topological magnon materials identified in this work. These materials exhibit a nontrivial $\mathbb{Z}_4$ inversion index when breaking into one of the magnetic subgroups (\textit{e.g.} $P\bar{1}$, $P2^\prime_1/c^\prime$, $C2^\prime/m^\prime$, \textit{etc.}). The index can indicate either gapless Weyl magnons or gapped magnon axion insulator states depending on the material's magnetic subgroup and interaction details.} 
\label{tab:magnon_materials} \\
\hline
\textbf{Category} & \textbf{Materials} \\
\hline
\endfirsthead

\hline
\textbf{Category} & \textbf{Materials} \\
\hline
\endhead

\hline
\endfoot

\hline

\textbf{I: Transition Metal Magnets} & \\
\textit{IA: Transition Metal Insulators} & $\alpha$-Fe$_2$O$_3$, CoO, MnTe$_2$, NiFe$_2$O$_4$, NiCr$_2$O$_4$, MnV$_2$O$_4$, CdYb$_2$S$_4$, CdYb$_2$Se$_4$, MnPb$_4$Sb$_6$S$_{14}$, FePb$_4$Sb$_6$S$_{14}$, Ba$_2$CoO$_2$Ag$_2$Se$_2$, Sr$_2$CoO$_2$Ag$_2$Se$_2$, Sr$_2$Fe$_3$S$_2$O$_3$, BaCoSO, Sr$_3$ZnIrO$_6$, Ca$_4$IrO$_6$, Ca$_3$LiRuO$_6$, Sr$_3$LiRuO$_6$, Sr$_3$NaRuO$_6$, SrFeO$_2$, Ca$_3$LiOsO$_6$, Ca$_2$MnGaO$_5$, CuSb$_2$O$_6$, Cr$_2$ReO$_6$, Ca$_2$Fe$_2$O$_5$, Mn$_3$TeO$_6$, FeTa$_2$O$_6$, GeNi$_2$O$_4$, LiMnAs, CsMnP, CsMnBi, RbMnAs, RbMn, RbMnP, KMnP, KMnAs, RbMnAs, RbMnBi \\
\hdashline
\textit{IB: Metallic TM Pnictogens and Chalcogens} & CrN, Li$_{0.5}$FeCr$_{1.5}$S$_4$, FeCr$_2$S$_4$, SrMnSb$_2$, CoNb$_3$S$_6$, CsCo$_2$Se$_2$, CaCo$_{1.86}$As$_2$, Sr$_2$Cr$_3$As$_2$O$_2$, CuSe$_2$O$_5$ \\
\hdashline
\textit{IC: Metal to Insulator Transition Compounds} & NiS$_2$, KCuMnS$_2$, USb \\
\hdashline
\textit{ID: Transition Metal Intermetallics} & MnPt$_{0.5}$Pd$_{0.5}$, Mn$_3$Pt, MnCoGe, Mn$_5$Si$_3$, Fe$_{0.7}$Mn$_{0.3}$, Ni$_{1.64}$Co$_{0.36}$Mn$_{1.28}$Ga$_{0.72}$, Mn$_3$Sn$_2$, PrMnSi$_2$, CaFe$_4$Al$_8$, FeGe, FeSn, FeSn$_2$, FeGe$_2$, Mn$_3$Cu$_{0.5}$Ge$_{0.5}$N, Mn$_3$GaN, Mn$_3$ZnN, Mn$_3$GaC, Mn$_3$CuN, Mn$_2$As, Fe$_2$As, Cr$_2$As, EuFe$_2$As$_2$ \\
\hline

\textbf{II: f-block Magnets} & \\
\textit{IIA: Insulating f-block Magnets} & UO$_2$, NpSe, NpS, DyOCl, HoP, La$_3$OsO$_7$, La$_{2.8}$Ca$_{0.2}$OsO$_7$, Cd$_2$Os$_2$O$_7$, Ho$_2$Ru$_2$O$_7$, Er$_2$Ru$_2$O$_7$, Dy$_3$Al$_5$O$_{12}$, Tb$_3$Al$_5$O$_{12}$, Ho$_3$Al$_5$O$_{12}$, Er$_3$Ga$_5$O$_{12}$, Dy$_3$Ga$_5$O$_{12}$, Tb$_3$Ga$_5$O$_{12}$, Ho$_3$Ga$_5$O$_{12}$, Ln$_3$Tr$_5$O$_{12}$, Tm$_2$Mn$_2$O$_7$, Ho$_2$CrSbO$_7$, Ho$_2$Ru$_2$O$_7$, Er$_2$Ti$_2$O$_7$, Gd$_2$Sn$_2$O$_7$, Er$_2$Pt$_2$O$_7$, Er$_2$Sn$_2$O$_7$, Gd$_2$Ti$_2$O$_7$, Nd$_2$Sn$_2$O$_7$, Nd$_2$Hf$_2$O$_7$, Nd$_2$Zr$_2$O$_7$, Nd$_2$ScNbO$_7$, Sm$_2$Ti$_2$O$_7$, Tb$_2$Sn$_2$O$_7$, Yb$_2$Ti$_2$O$_7$, Yb$_2$Sn$_2$O$_7$ \\
\hdashline
\textit{IIB: Metallic f-block Pnictogens and Chalcogens} & UP, USb$_2$, UP$_2$, UGeS, UGeTe, NpBi, NpTe, NdCoAsO, LaCrAsO, CeCo$_2$P$_2$, CeSbTe \\
\hdashline
\textit{IIC: f-block Intermetallics} & Ho(Co$_{0.66}$Ga$_{0.33}$)$_2$, CeIr(In$_{0.97}$Cd$_{0.03}$)$_5$, ErNiGe, NdCo$_2$, GdMg, Pr$_2$Pd$_2$In, NdZn, Ho$_3$NiGe$_2$, Pr$_3$CoGe$_2$, Tb$_{0.6}$Y$_{0.4}$RhIn$_5$, NdMg, NdPt, TbPd$_{2.05}$Sn$_{0.95}$, Ho$_3$Ge$_4$, NdNiMg$_{15}$, Er$_3$Ge$_4$, Ce$_2$Ni$_3$Ge$_5$, HoRh, Yb$_2$Pd(In$_{0.4}$Sn$_{0.6}$), NdPd$_5$Al$_2$, ErFe$_2$Si$_2$, NdScSiC$_{0.5}$H$_{0.2}$, UNiGa$_5$, UPd$_2$Ge$_2$, URh$_3$Si$_5$, NpNiGa$_5$, U$_2$Pd$_{2.35}$Sn$_{0.65}$, ErMn$_2$Ge$_2$, YMn$_2$Si$_2$, YMn$_2$Ge$_2$, EuMn$_2$Si$_2$, CeMn$_2$Si$_2$, NdMn$_2$Si$_2$, PrMn$_2$Si$_2$, ErMn$_2$Ge$_2$, TbMn$_2$Si$_2$, DyCu, TbPt, TbPt$_{0.8}$Cu$_{0.2}$, NdSi, DyPt, TmNi, PrSi, NdNi$_{0.6}$Cu$_{0.4}$, HoNi, HoPt, ErPt, TmPt, Tb$_2$CoGa$_8$, Dy$_2$CoGa$_8$, Nd$_2$RhIn$_8$, U$_2$Rh$_2$Sn, U$_2$Ni$_2$Sn, CeRh$_2$Si$_2$, CeRu$_2$Al$_{10}$, U$_2$Ni$_2$In, YbCo$_2$Si$_2$ \\
\hline

\textbf{III: Structurally Distinct} & \\
\textit{IIIA: Perovskite oxides and their derivatives} & BiCrO$_3$, TbCr$_{0.5}$Mn$_{0.5}$O$_3$, Lu$_{0.6}$Mn$_{0.4}$MnO$_3$, Pb$_{0.7}$Bi$_{0.3}$Fe$_{0.762}$W$_{0.231}$O$_3$, Pb$_{0.8}$Bi$_{0.2}$Fe$_{0.728}$W$_{0.264}$O$_3$, Nd$_2$CuO$_4$, Sr$_2$IrO$_4$, Nd$_2$NiO$_4$, Ca$_2$RuO$_4$, La$_2$NiO$_4$, LaSr$_3$Fe$_3$O$_9$, CaCu$_3$Fe$_2$Sb$_2$O$_{12}$, Sr$_2$CoOsO$_6$, Sr$_2$FeOsO$_6$, Cu$_3$Ni$_2$SbO$_6$, Bi$_2$RuMnO$_7$, NdFeO$_3$, CeFeO$_3$, TbFeO$_3$, SmFeO$_3$, NaOsO$_3$, LaCrO$_3$, YCrO$_3$, LaMnO$_3$, ErCrO$_3$, TmCrO$_3$, YRuO$_3$, PrMnO$_3$, Pr$_{0.95}$K$_{0.05}$MnO$_3$, NdMnO$_3$, KMnF$_3$, NdMnO$_3$, (CH$_3$NH$_3$)(Co(COOH)$_3$), Ho$_{0.2}$Bi$_{0.8}$FeO$_3$, Ho$_{0.15}$Bi$_{0.85}$FeO$_3$, La$_{0.875}$Ba$_{0.125}$Mn$_{0.875}$Ti$_{0.125}$O$_3$, La$_{0.90}$Ba$_{0.10}$Mn$_{0.90}$Ti$_{0.10}$O$_3$, La$_{0.95}$Ba$_{0.05}$Mn$_{0.95}$Ti$_{0.05}$O$_3$, La$_{0.95}$Ba$_{0.05}$MnO$_3$, LaMnO$_3$, YCr$_{0.5}$Mn$_{0.5}$O$_3$, SmFeO$_3$, SrRuO$_3$, TbCrO$_3$, DyCrO$_3$, TeNiO$_3$, YVO$_3$, LaSrFeO$_4$, Nd$_2$CuO$_4$, Pr$_2$CuO$_4$, LaSrFeO$_4$, LaCaFeO$_4$, LaBaFeO$_4$, La$_{0.75}$Bi$_{0.25}$Fe$_{0.5}$Cr$_{0.5}$O$_3$, LaCrO$_3$, CeFeO$_3$, InCrO$_3$, TlCrO$_3$, ScCrO$_3$, La$_2$NiO$_4$, Nd$_2$NiO$_4$, La$_2$CoO$_4$, Gd$_2$CuO$_4$, Sm$_2$CuO$_4$, Eu$_2$CuO$_4$, Bi$_{0.8}$La$_{0.2}$Fe$_{0.5}$Mn$_{0.5}$O$_3$, PrCrO$_3$, SmCrO$_3$, NdMn$_{0.8}$Fe$_{0.2}$O$_3$, Bi$_{0.8}$La$_{0.2}$Fe$_{0.5}$Mn$_{0.5}$O$_3$, PrCrO$_3$, SmCrO$_3$, NdMn$_{0.8}$Fe$_{0.2}$O$_3$, Rb$_2$Fe$_2$O(AsO$_4$)$_2$, NdMnO$_3$, NdMn$_{0.8}$Fe$_{0.2}$O$_3$, Pr$_{0.5}$Sr$_{0.5}$CoO$_3$, Pr$_{0.5}$Sr$_{0.4}$Ba$_{0.1}$CoO$_3$, Pr$_{0.5}$Sr$_{0.5}$MnO$_3$, (Tm$_{0.7}$Mn$_{0.3}$)MnO$_3$, (Ho$_{0.8}$Mn$_{0.2}$)MnO$_3$, Tb$_{0.55}$Sr$_{0.45}$MnO$_3$, Tb$_{0.55}$Sr$_{0.45}$MnO$_3$, SmCrO$_3$, TbFeO$_3$, Sc$_2$NiMnO$_6$, La$_2$CoPtO$_6$, Ca$_2$Fe$_{0.875}$Cr$_{0.125}$GaO$_5$ \\
\hdashline
\textit{IIIB: Halides and oxyhalides} & KNiF$_3$, KMnF$_3$, FeF$_3$, LiCoF$_4$, NaMnF$_4$, Na$_2$NiFeF$_7$, CsMn$_2$F$_6$, Fe$_2$F$_5$(H$_2$O)$_2$, Cr$_2$F$_5$, CsMnF$_4$, TlMnF$_4$, Na$_2$NiCrF$_7$, CsCoCl$_3$(D$_2$O)$_2$, CsNiF$_3$, SrFeO$_2$F, La$_2$NiO$_3$F$_2$, La$_{0.5}$Sr$_{0.5}$FeO$_{0.5}$F$_{0.5}$, Mn$_2$SeO$_3$F$_2$, Cu$_3$Mg(OD)$_6$Br$_2$, La$_2$NiO$_3$F$_{1.93}$ \\
\hdashline
\textit{IIIC: Polyatomic oxides (Sulfates, Phosphates, Carbonates, Vanadates, Germanates, Silicates)} & NiSO$_4$, FeSO$_4$, CoSO$_4$, FeSO$_4$F, FeOH$_4$, Li$_2$Fe(SO$_4$)$_2$, NaFeSO$_4$F, NaCoSO$_4$F, Co$_3$(PO$_4$)$_2$, CuFe$_2$(P$_2$O$_7$)$_2$, Fe$_2$MnBO$_5$, AgMnVO$_4$, VPO$_4$, Na$_3$Co(CO$_3$)$_2$Cl, Na$_2$BaMn(VO$_4$)$_2$, MnCO$_3$, NiCO$_3$, CoCO$_3$, Cu$_3$Y(SeO$_3$)$_2$O$_2$Cl, Cu$_3$Bi(SeO$_3$)$_2$O$_2$Br, (NH$_2$(CH$_3$)$_2$)(FeMn(HCOO)$_6$), (CH$_3$NH$_3$)Co(COOH)$_3$, (NH$_2$(CH$_3$)$_2$)(FeCo(HCOO)$_6$), NH$_4$FeCl$_2$(HCOO), [C(ND$_2$)$_3$]Mn(DCOO)$_3$, KFe$_3$(SO$_4$)$_2$(OH)$_6$, NaFe$_3$(SO$_4$)$_2$(OH)$_6$, AgFe$_3$(SO$_4$)$_2$(OD)$_6$, FeBO$_3$, CoFePO$_5$, NaFePO$_4$, Na$_2$BaFe(VO$_4$)$_2$, LaMn$_3$V$_4$O$_{12}$, ZrCo$_2$Ge$_4$O$_{12}$, CeCo$_2$Ge$_4$O$_{12}$, CeMnCoGe$_4$O$_{12}$, ZrMn$_2$Ge$_4$O$_{12}$, GdFeZnGe$_4$O$_{12}$, ErFeCuGe$_4$O$_{12}$, NaCeGe$_2$O$_6$, Fe$_4$Si$_2$Sn$_7$O$_{16}$, Mn$_2$SiO$_4$, Mn$_2$GeO$_4$, CuCl(C$_4$H$_4$N$_2$)$_2$(BF$_4$), CuBr(C$_4$H$_4$N$_2$)$_2$(BF$_4$) \\

\end{longtable}
